Optimistic Natural Policy Gradient: a Simple Efficient Policy Optimization Framework for Online RL

While policy optimization algorithms have played an important role in recent empirical success of Reinforcement Learning (RL), the existing theoretical understanding of policy optimization remains rather limited -- they are either restricted to tabular MDPs or suffer from highly suboptimal sample complexity, especial in online RL where exploration is necessary. This paper proposes a simple efficient policy optimization framework -- Optimistic NPG for online RL. Optimistic NPG can be viewed as a simple combination of the classic natural policy gradient (NPG) algorithm [Kakade, 2001] with optimistic policy evaluation subroutines to encourage exploration. For $d$-dimensional linear MDPs, Optimistic NPG is computationally efficient, and learns an $\varepsilon$-optimal policy within $\tilde{O}(d^2/\varepsilon^3)$ samples, which is the first computationally efficient algorithm whose sample complexity has the optimal dimension dependence $\tilde{\Theta}(d^2)$. It also improves over state-of-the-art results of policy optimization algorithms [Zanette et al., 2021] by a factor of $d$. In the realm of general function approximation, which subsumes linear MDPs, Optimistic NPG, to our best knowledge, stands as the first policy optimization algorithm that achieves polynomial sample complexity for learning near-optimal policies.

==> legacy/abstract.tex <==



\begin{abstract}
We propose a computationally efficient, model-free, policy optimization algorithm---\oppo~for RL of linear MDPs in  the online, episodic, finite-horizon setting.
\oppo~can be viewed as an optimistic version of the classic natural policy gradient (NPG) algorithm \citep{kakade2001natural} because it utilizes bonus-induced optimism to encourage exploration.  
We prove that \oppo~learns an $\epsilon$-optimal policy for any  $d$-dimensional linear MDPs within $\tilde{\cO}(d^2/\epsilon^3)$ samples, which improves over the SOTA results of policy optimization algorithms \citep{zanette2021cautiously} by a factor of $d$. Moreover, to our knowledge, it is the first computationally efficient algorithm whose sample complexity has the optimal  
dimension dependence $\tilde{\Theta}(d^2)$.
\end{abstract}



% \begin{abstract}
% We propose a new model-free, policy optimization method 
% for linear MDPs and analyze its behavior in the online, episodic, fixed horizon setting.
% The algorithm considered is a variation of Politex, where, crucially, in the policy
% evaluation step, which is performed with LSPE, a well-chosen bonus is introduced.
% We show that for constant precision, after $O(d^2)$ episodes, this algorithm 
% returns a near-optimal precision, where $d$ is the dimension
% of the feature space. 
% This bound shaves off a factor of $d$ from the previous state-of-the-art.
% Our algorithm is model-free, computationally efficient and in particular it does not need
% an optimistic planner and as such it is easy to adopt it to use neural networks in place of
% linear function approximation. To our best knowledge, this is the first policy optimization
% algorithm that is proven to have polynomial sample complexity for linear MDPs.
% \end{abstract}

==> legacy/app.tex <==

\section{Proofs for Section \ref{sec:proof-sketch}}
\label{app:linear}

\subsection{Proof of Lemma \ref{lem:pi-diff}}
Lemma \ref{lem:pi-diff} is an immediate consequence of Lemma 4.2 in \citep{cai2020provably} or Lemma 1 in \citep{shani2020optimistic}.

\subsection{Proof of Lemma \ref{lem:opt}}
Let us consider a fixed pair  $(k,h)\in[K]\times[H]$. Recall $\oQ_h^k$ is defined as 
$$
\oQ_h^k(s,a)= {\rm Truncate}_{[0,H-h+1]}\big( \langle \hat \theta_h^k, \phi_h(s,a)\rangle + b_h^k(s,a)\big), 
$$
where 
\begin{equation*}
\hat \theta_h^k =  \argmin_{\theta}
\hspace{-6mm}\sum_{(s_h,a_h,r_h,s_{h+1})\in\cD_h^k} \bigg(\phi_h(s_h,a_h)\trans\theta  -  r_h - \oV_{h+1}^k(s_{h+1}) \bigg)^2 + \lambda \|\theta\|_2^2,
\end{equation*}
\begin{equation*}
    b_h^k(s,a) = \alpha\times \|\phi_h(s,a)\|_{(\Sigma_h^k +\lambda \I_{d\times d})^{-1} }, \quad \text{and} \quad \Sigma_h^k =\sum_{(s_h,a_h)\in\cD_h^k} \phi(s_h,a_h)(\phi(s_h,a_h))\trans.
\end{equation*}
By the standard linear completeness property of linear MDPs \cite{jin2020provably}, there exists $\theta_h^k$ such that 
$\|\theta_h^k\|_2\le H\sqrt{d}$ and 
$$
\langle \phi_h(s,a), \theta_h^k\rangle = R_h(s,a) + \E_{s'\sim\P(\cdot \mid s,a)}\left[ \oV_{h+1}^k(s')\right] \quad \text{for all } (s,a)\in\cS\times\cA.
$$
Therefore, to prove Lemma \ref{lem:opt}, it suffices to show that  for all $(s,a)$
$$
\left|\langle \phi_h(s,a),\theta_h^k -
\hat\theta_h^k\rangle\right|\le b_h^k(s,a).
$$
To condense notations, denote by $\{(s_h^i,a_h^i,r_h^i,s_{h+1}^i)\}_{i=1}^M$ the tuples in $\cD_h^k$. 
By the definition of ridge regression,
\begin{align*}
   \MoveEqLeft \left|\langle \phi_h(s,a),\hat\theta_h^k-\theta_h^k \rangle\right| \\
=&\bigg|\bigg\langle \phi_h(s,a)~,~(\Sigma_h^k+\lambda \I_{d\times d})^{-1}\left(\sum_{i=1}^M\phi_h(s_h^i,a_h^i) \left(  r_h^i + \oV_{h+1}^k(s_{h+1}^i)-\phi_h(s_h^i,a_h^i)\trans\theta^k_h\right)-\lambda \theta_h^k\right)\bigg\rangle\bigg|\\
\le & \|\phi_h(s,a)\|_{(\Sigma_h^k +\lambda \I_{d\times d})^{-1} } \times \left(\left\|\sum_{i=1}^M\phi_h(s_h^i,a_h^i) \left(  r_h^i + \oV_{h+1}^k(s_{h+1}^i)-\phi_h(s_h^i,a_h^i)\trans\theta^k_h\right)\right\|_{(\Sigma_h^k +\lambda \I_{d\times d})^{-1} }+H\sqrt{d} \right),
\end{align*}
where the inequality follows from 
$ \| \lambda \theta_h^k\|_{(\Sigma_h^k +\lambda \I_{d\times d})^{-1} }\le \sqrt{\lambda}\|\theta_h^k\|_2 \le H\sqrt{d}.
$
It remains to bound the first term in the bracket.
Now here comes the key observation that helps shave off the $\sqrt{d}$ factor from the bonus.
\begin{observation}\label{obs:ind}
$\cD_h^k$ and $\oV_{h+1}^k$ are independent conditioning on $\pi^{t_k}$ where $t_k$ denotes the index of the last iteration of collecting fresh data before the $k\th$ iteration.
\end{observation}
To see why, recall that after obtaining $\cD^{t_k}$ Algorithm \ref{alg:lspe} splits it evenly into $H$ disjoint subsets $\{\cD_h^{t_k}\}_{h=1}^H$ and then only uses
$\{\cD_{h'}^{t_k}\}_{h'=h+1}^H$ for evaluating and improving $\{\pi_{h'}^l\}_{h'=h+1}^H$ for $l\in[t_k,t_k+m-1]$. As a result,  $\{\oV_{h+1}^l\}_{l=t_k}^{t_k+m-1}$ (including $\oV_{h+1}^k$) is independent of $\cD_h^{t_k}=\cD_h^k$ conditioning on $\pi^{t_k}$. 
By the concentration of self-normalized processes \citep{abbasi2011improved}, we conclude that with probability at least $1-\delta$: for all $(k,h)\in[K]\times[H]$
$$
\left\|\sum_{i=1}^M\phi_h(s_h^i,a_h^i) \left(  r_h^i + \oV_{h+1}^k(s_{h+1}^i)-\phi_h(s_h^i,a_h^i)\trans\theta^k_h\right)\right\|_{(\Sigma_h^k +\lambda \I_{d\times d})^{-1} }
\le \cO\left(H\sqrt{d\log(MKH/\delta)}\right).
$$

\subsection{Proof of Lemma \ref{lem:pi-close}}

We first introduce the following two auxiliary lemmas about the lipschitzness continuity of softmax paraterization.  




\begin{lemma}\label{lem:policy-stability}
There exists an absolute constant $c>0$ such that for any policy $\pi,\hat\pi$ satisfying $\hat\pi_h(a\mid s) \propto \pi_h(a\mid s)\times \exp(L_h(s,a))$ where $\{L_h(s,a)\}_{h\in[H]}$ is set of  functions from $\cS\times\cA$ to $[-1/H,1/H]$, we have that for any $\tau_H:=(s_1,a_1,\ldots,s_H,a_H)\in(\cS\times\cA)^H$:
$$
\P^{\hat\pi}(\tau_H) 
\le c\times \P^\pi(\tau_H).
$$
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:policy-stability}]
By using the relation between $\pi$ and $\hat\pi$ and the normalization property of policy $\pi$, we have that for any $(h,s,a)$:
\begin{align*}
\hat\pi_h(a\mid s)
& = \frac{\pi_h(a\mid s) \times \exp(L_h(s,a))}{\sum_{a'} \pi_h(a'\mid s) \times \exp(L_h(s,a'))} \\
& \le 
\frac{\pi_h(a\mid s) \times \exp(1/H)}{\sum_{a'} \pi_h(a'\mid s) \exp(-1/H) } \\
& = \pi_h(a\mid s) \times \exp(2/H)
\le \pi_h(a\mid s) \times \left(1+\frac{\cO(1)}{H}\right).
\end{align*}
Therefore, for any 
$\tau_H:=(s_1,a_1,\ldots,s_H,a_H)$
\begin{align*}
\P^{\hat\pi}(\tau_H) = &  \left(\prod_{h=1}^{H-1} \P_h(s_{h+1}\mid s_h,a_h)\right)
\times 
\left(\prod_{h=1}^{H} \hat\pi_h(a_h\mid s_h)\right)\\
\le  & \left(\prod_{h=1}^{H-1} \P_h(s_{h+1}\mid s_h,a_h)\right)
\times 
\left(\prod_{h=1}^{H}
\pi_h(a_h\mid s_h)\right)\times \left(1+\frac{\cO(1)}{H}\right)^H \\
= &\cO(1) \times 
\left(\prod_{h=1}^{H-1} \P_h(s_{h+1}\mid s_h,a_h)\right)
\times 
\left(\prod_{h=1}^{H}
\pi_h(a_h\mid s_h)\right)
= \cO(1) \times 
\P^{\pi}(\tau_H).
\end{align*}
\end{proof}


\begin{lemma}\label{lem:transfer}
Let $\mu,\nu$ be two probability densities defined over $\cX$ such that 
$\|\mu/\nu\|_\infty \le \alpha$, then we have that  for any function  $f:\cX\rightarrow \R^+$, $\E_\mu[f(x)] \le \alpha \E_\nu[f(x)]$.
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:transfer}]
By definition, $\E_\mu[f(x)] = \int_x f(x) \mu(x)dx \le \int_x f(x) (\alpha\nu(x))dx = \alpha \E_\nu[f(x)].$
\end{proof}


By the update rule of NPG, we have 
$$
\pi^{k}_h(\cdot \mid s) \propto \pi^{t_k}_h(\cdot \mid s)\times \exp\left( \eta\sum_{i=t_k}^{k-1} \oQ_h^i(s,\cdot) \right).
$$
Since we choose $\eta$ and $m$ such that $\eta m \le 1/H^2$, 
$$
\left|\eta\sum_{i=t_k}^{k-1} \oQ_h^i(s,\cdot)\right|\le \eta (k-t_k)H\le \eta m H \le 1/H.
$$
Therefore, by invoking Lemma \ref{lem:policy-stability} with $\hat\pi=\pi^k$ and $\pi=\pi^{t_k}$, we have that for any $\tau_H\in(\cS\times\cA)^H$:
$$
\P^{\pi^k}(\tau_H) 
\le c\times \P^{\pi^{t_k}}(\tau_H).
$$
By further invoking Lemma \ref{lem:transfer} with $\cX=(\cS\times\cA)^H$, $\mu=\P^{\pi^k}$ and $\nu=\P^{\pi^{t_k}}$, we obtain that for any function $f:\cS\times\cA\rightarrow \R^+$:
$$
\E_{\pi^k}[f(s_h,a_h)] = \cO\left(
\E_{\pi^{t_k}}[f(s_h,a_h)]\right).
$$
Similarly, we can show 
$\E_{\pi^{t_k}}[f(s_h,a_h)] = \cO\left(\E_{\pi^k}[f(s_h,a_h)]\right)$, which completes the proof of Lemma \ref{lem:pi-close}.


\subsection{Proof of Lemma \ref{lem:on-policy-bonus}}

To simplify notations, denote  $\phi^i_h :=\phi_h(s_h^i,a_h^i)$.
For the technical purpose of applying martingale concentration, we additionally define the intermediate empirical covariance matrices: $\Sigma_h^n=\sum_{i=1}^{n-1} \phi_h^i (\phi_h^i)\trans$, for $n\in[N]$. 
We have that with probability at least $1-\delta$,
\begin{equation}
    \begin{aligned}
     \MoveEqLeft \E_{(s_h,a_h)\sim\pi}\big[\|\phi_h(s_h,a_h)\|_{(\Sigma_h+ \lambda  \I_{d\times d})^{-1}}\big] \\ &\le \frac{1}{N}\sum_{n=1}^N  \E_{(s_h,a_h)\sim\pi}\big[\|\phi_h(s_h,a_h)\|_{(\Sigma_h^n+ \lambda  \I_{d\times d})^{-1}}\big] \\
     & \le \frac{1}{N}\sum_{n=1}^N  \|\phi_h^n\|_{(\Sigma_h^n+ \lambda  \I_{d\times d})^{-1}} + \cO\left( \sqrt{\frac{\log(1/\delta)}{N}}\right)\\
     & \le \cO\left(\sqrt{\frac{d\log N}{N}}\right) + \cO\left( \sqrt{\frac{\log(1/\delta)}{N}}\right), 
    \end{aligned}
\end{equation}
where the first inequality uses $\Sigma_h^n \preceq \Sigma_h$,  the second one uses Azuma-Hoeffding inequality with $\lambda =1$, and the last one uses Cauchy–Schwarz inequality and the the standard elliptical potential argument.


\section{Proofs for Section \ref{sec:tab}}
\label{app:tab}



\subsection{Proof of Lemma \ref{lem:opt-tabular}} Let us consider a fixed pair  $(k,h)\in[K]\times[H]$. Recall $\oQ_h^k$ is defined as 
\begin{equation*}
    \oQ_h^k(s,a)= \min\big\{H-h+1,~
    \E_{s'\sim\hat\P_h^k (s,a)}[ \oV_{h+1}^k(s')]+\hat R_h^k(s,a)+ b_h^k(s,a)\big\}
\end{equation*}
 where  $\hat\P_h^k$ and $\hat\R_h^k$ are the empirical estimates of transition and reward at step $h$ from $\cD_h^k$, and 
 $b_h^k(s,a)=\alpha({J_h^k(s,a)+1})^{-1/2}$ with $J_h^k(s,a)=\sum_{(s_h,a_h)\in\cD_h^k}\mathbf{1}((s_h,a_h)=(s,a))$. Therefore, to prove Lemma \ref{lem:opt-tabular}, it suffices to show that  for all $(s,a)$
$$
\left|\left(\E_{s'\sim\hat\P_h^k (s,a)}[ \oV_{h+1}^k(s')] - 
\E_{s'\sim\P_h (s,a)}[ \oV_{h+1}^k(s')]\right)+\left(\hat R_h^k(s,a) - R_h(s,a)\right)
\right|\le b_h^k(s,a).
$$
By observation \ref{obs:ind}, we know    $\{\oV_{h+1}^l\}_{l=t_k}^{t_k+m-1}$ is independent of $\cD_h^{t_k}=\cD_h^k$ conditioning on $\pi^{t_k}$, which implies $\oV_{h+1}^k$ is independent of $\hat\P_h^k$. Therefore, by Azuma-Hoeffding inequality and standard union bound, we conclude that with probability at least $1-\delta$: for all $(k,h,s,a)\in[K]\times[H]\times\cS\times\cA$, 
$$
\left|\left(\E_{s'\sim\hat\P_h^k (s,a)}[ \oV_{h+1}^k(s')] - 
\E_{s'\sim\P_h (s,a)}[ \oV_{h+1}^k(s')]\right)+\left(\hat R_h^k(s,a) - R_h(s,a)\right)
\right|\le \cO\left(H\sqrt{\frac{\log(KHSA/\delta)}{J_h^k(s,a)+1}}\right).
$$


\subsection{Proof of Lemma \ref{lem:on-policy-bonus-tabular}}For the technical purpose of performing martingale concentration, we introduce the notion of  intermediate counters: $J_h^n(s,a)=\sum_{i=1}^{n-1}  \mathbf{1}((s_h^i,a_h^i)=(s,a))$, for $n\in[N]$. 
We have that with probability at least $1-\delta$,
\begin{equation}
    \begin{aligned}
     \MoveEqLeft   \E_{(s_h,a_h)\sim\pi}\left[\sqrt{\frac{1}{J_h(s,a)+1}}\right]  \\ &\le \frac{1}{N}\sum_{n=1}^N    \E_{(s_h,a_h)\sim\pi}\left[\sqrt{\frac{1}{J_h^n(s,a)+1}}\right]  \\
     & \le \frac{1}{N}\sum_{n=1}^N  \sqrt{\frac{1}{J_h^n(s_h^n,a_h^n)+1}}+ \cO\left( \sqrt{\frac{\log(1/\delta)}{N}}\right)\\
     & \le \cO\left(\sqrt{\frac{SA\log N}{N}}\right) + \cO\left( \sqrt{\frac{\log(1/\delta)}{N}}\right), 
    \end{aligned}
\end{equation}
where the first inequality uses $J_h^n(s,a) \le J_h(s,a)$ for all $(s,a)\in\cS\times\cA$,  the second one uses Azuma-Hoeffding inequality, and the last one follows the standard pigeon-hole argument.


==> legacy/conc.tex <==
%!TEX root =  main.tex

\section{Conclusions}
We proposed a computationally efficient, model-free, policy optimization
%We proposed a new model-free, policy optimization
algorithm---\oppo~for linear MDPs and analyzed its behavior in the online, episodic, fixed horizon setting.
In terms of algorithmic design, it is not only considerably simpler but also more closely resembles  the empirical policy optimization algorithms (e.g., PPO, TRPO) than the previous theoretical algorithms. 
In terms of sample efficiency, it 
improves over the SOTA policy optimization algorithm by a factor of $d$ for RL of $d$-dimensional linear MDPs. Moreover, to our knowledge, it is the first computationally efficient algorithm to achieve the optimal dimension dependence. For future research, we believe the following directions are worth exploring.
\begin{itemize}
    \item Despite the optimal dependence on dimension $d$, the current sample complexity of \oppo~is worse than the optimal rate by a factor of $1/\epsilon$. It remains unclear to us how to shave off this $1/\epsilon$ factor to achieve the optimal rate.
    \item In this work we restrict our attention to the setting of linear MDPs. It is natural to ask whether one can generalize the current algorithmic design and analysis to deal with general function approximation under mild assumptions.
    \item \oppo~features an on-policy mechanism to collect fresh data periodically, which plays a key role in achieving the optimal dimension dependence. 
    Since this mechanism is not restrictively designed  for  linear MDPs, we believe it could  potentially be used to obtain sharper rates in other RL problems.
\end{itemize}




==> legacy/intro.tex <==
%!TEX root =  main.tex

\section{Introduction}

Policy optimization algorithms \cite{schulman2017proximal,schulman2015trust} with neural network function approximation have played an important rule in recent empirical success of  reinforcement learning (RL), such as robotics \cite{finn2016guided}, games \cite{berner2019dota} and large language models \cite{chatgpt}. 
Motivated by the empirical success, the theory community made a large effort to 
design provably efficient policy optimization algorithms that work in the presence of linear function approximation \citep{agarwal2021theory,bhandari2019global,liu2019neural,neu2017unified,abbasi2019politex,agarwal2020pc,zanette2021cautiously,shani2020optimistic,cai2020provably}.
Early works focused on proving that  policy optimization algorithms are capable to learn near-optimal policies using a polynomial number of samples under certain reachability (coverage) assumptions.
 \citep[e.g.,][]{agarwal2021theory,bhandari2019global,liu2019neural,neu2017unified,abbasi2019politex}.
While this was good for laying down the foundations for future work,  
the reachability assumptions  basically imply that the state space is already well-explored or rather easy to explore, which avoids the challenge of performing strategic exploration --- one of the central problems in both empirical and theoretical RL. 
 To address this limitation,  later works \citep{agarwal2020pc,zanette2021cautiously}  proposed  policy optimization algorithms that enjoy polynomial sample complexity guarantee without making any reachability assumption, but at the cost of either  complicating the algorithm design (and analysis) with  various  tricks or getting highly suboptimal sample complexity guarantees. 
 For example, the PC-PG algorithm \cite{agarwal2020pc}, which, to our knowledge was the first policy optimization algorithm for learning linear MDPs without reachability assumption, 
 requires  $\tilde{\cO}(\poly(d)/\epsilon^{11})$ samples to learn an $\epsilon$-optimal policy for $d$-dimensional linear MDPs. 
That $\tilde{\cO}(1/\epsilon^{11})$ samples were necessary for this task 
 is highly unlikely.
 Indeed,  \citet{zanette2021cautiously} greatly improved this sample complexity to $\tilde{\cO}(d^3/\epsilon^3)$ at the cost of considerably  complicating the algorithm design and the analysis. 

  
 In this paper, we attempt to answer the following question: \begin{center}
    \textsl{Can we design a \textbf{simpler} policy optimization algorithm with \textbf{sharper} sample complexity guarantee\\
    in the \textbf{exploration} setting?}
 \end{center}
We answer this question affirmatively by making the following contributions:
\begin{itemize}
    \item \textbf{Sharper rate.} We propose a computationally efficient policy optimization algorithm---\oppo~with sample complexity  
    \[
    \tilde{\cO}(d^2/\epsilon^3)
    \]
     for learning an $\epsilon$-optimal policy in 
    an online fashion while interacting with a 
    $d$-dimensional
    linear MDPs.
    This result improves over the best previous one \citep{zanette2021cautiously} in  policy optimization by a factor of $d$. 
    Moreover, to our knowledge, this is the first computationally efficient algorithm to achieve the optimal quadratic dimension dependence. 
    Before moving on, we remark that previous FQI-style algorithms \citep{zanette2020learning,jin2021bellman} achieve the optimal 
     sample complexity \citep{zanette2020learning} \[
     \tilde{\Theta}(d^2/\epsilon^2)
     \]
      but they are   computationally \emph{inefficient} due to the mechanism of global optimism  in  %\newpage 
    their   algorithm design. 
    Several very recent works
    \citep{he2022nearly,agarwal2022vo,wagenmaker2022reward} achieve the sample complexity 
    \[
    \tilde{\cO}(d^2/\epsilon^2+d^{\ge 4}/\epsilon)
    \]
    using computationally efficient algorithms. 
    Compared to this work, the above rate has worse dependence on $d$ and better dependence on $\epsilon$.
    Nonetheless, our result is better in the practically important regime where the feature dimension $d$ is typically very large and the target accuracy $\epsilon$ is not too small. 
    To summarize, the sample complexity of \oppo~strictly improves over the best existing policy optimization algorithms and is not dominated by that of any existing computationally efficient algorithm.
    
     \item \textbf{Simple on-policy algorithm.} 
     At a high level, \oppo~is almost an \emph{on-policy} version of natural policy gradient (NPG) \citep{kakade2001natural} 
     with Boltzmann policies that use linear function approximation 
     for optimistic action-value estimates. 
     By ``on-policy'', we mean the transition-reward data used to improve the current policy are obtained exactly by executing the current policy.
	However, the algorithm has a tuneable parameter (denoted by $m$ in Algorithm \ref{alg:oppo}) that allows it to reuse data sampled from 
	earlier policies. 
	By using such data, the algorithm becomes \emph{off-policy}.
	The optimal choice of the tuneable parameter is dictated by theoretical arguments.
	Interestingly, our analysis shows that 
	even the purely on-policy version of the algorithm (i.e., set $m=1$ in Algorithm \ref{alg:oppo}) enjoys
	a well-controlled sample complexity of $\tilde{\cO}(d^2/\epsilon^4)$.
% 	It is notable, that the algorithm can be shown to have polynomial sample complexity
% 	in the on-policy case; 
	To the best of our knowledge, this is the first time an on-policy 
	method is shown to have polynomial sample complexity in the exploration setting, given that all previous policy optimization or Q-learning style or model-based algorithms \citep[e.g.,][etc]{jin2020provably,zanette2020learning,zanette2021cautiously,agarwal2020pc,cai2020provably,shani2020optimistic}  are off-policy.  
 \item \textbf{New proof techniques.} To achieve the improved rate, we introduce several  new ideas in the proof, including but not limited to  (a) exploiting the softmax
parameterization of the policies to reuse data and improve sample efficiency (Lemma 3), (b) controlling \emph{on-policy} uncertainty  (Lemma 4) instead of cumulative uncertainty as in previous off-policy works, and  (c) using a bonus term that is smaller than those in previous works by a factor of $\sqrt{d}$ (see Lemma 2 and the discussions below).

  
	% To achieve this result, our paper introduces
	% \emph{new proof techniques}, avoiding 
	%  the ellipsoidal potential argument 
	%  that is at the heart of previous analyses 
	%   \citep[e.g.,][]{shani2020optimistic,cai2020provably,agarwal2020pc,zanette2021cautiously}
	%   and which eventually requires the use of (essentially) \emph{all} past data, which is less 
	%   sensible when it comes to ``model-based'' approaches (where the data is the model, essentially, like
	%   in FQI), but makes less sense in a policy optimization setting.
	% Nevertheless, we also consider a general version of the algorithm that allows the use of past data (i.e., set $m>1$ in Algorithm \ref{alg:oppo})
	% and in fact we show that using \emph{some amount} of past data leads to the improved upper bound
	% as far as the
	%  dependence on $\epsilon$ is considered. 
	%  The rational here is that
	%  the accuracy of the action-value estimates can be improved
	%   using data generated from \emph{recent} policies.
	% However, our analysis suggests that this only holds to some limit:
	% less recent policies may generate a vastly 
	% different distribution over the state space
	% (cf. Lemma \ref{lem:pi-close}), which makes such data less useful. 
	% (Note that bias plays no role here, due to our assumption that the MDP belongs to the family 
	% of linear MDPs with a known feature map.)
	% That using some amount of past data may be beneficial is intuitive and has been 
	% part of the design of many empirically successful policy optimization algorithms, 
	% such as   PPO
 %     \citep{schulman2017proximal}, TRPO \citep{schulman2015trust} and MPO \citep{abdolmaleki2018maximum}.


     
%      are on-policy, most existing theoretical works \citep[e.g.,][]{shani2020optimistic,cai2020provably,agarwal2020pc,zanette2021cautiously}  are inherently off-policy because they evaluate the current policy by using the data collected from  historical policies, for their technical purpose of utilizing elliptical potential arguments in proofs. 
%     In this sense, \oppo~is  more similar to the empirical policy optimization algorithms widely used in practice, and therefore requires different proof techniques from previous off-policy theory works.
\end{itemize}


\subsection{Related works}
 
Since this paper studies policy optimization algorithms in the setting of linear MDPs, below we  restrict our focus to previous theoretical works on either  policy optimization or linear MDPs.


 \paragraph{Policy optimization.}
This work is inspired by and  builds upon two recent works \citep{shani2020optimistic,cai2020provably} that combine NPG with bonus-based optimism to handle exploration. 
In terms of algorithmic design, this paper (\oppo) utilizes on-policy fresh data for value estimation while \citet{shani2020optimistic,cai2020provably} are off-policy and reuse \emph{all} the historical data.
In terms of theoretical guarantees, \citet{shani2020optimistic} and \citet{cai2020provably} only study tabular MDPs and  linear mixture MDPs \citep{zhou2021nearly} respectively, while this paper considers the more challenging setting of linear MDPs \citep{jin2020provably} (in our view, linear MDPs are more challenging as there the number of model parameters scale with the number of states).
 We remark that due to some subtle technical challenge, so far it still remains unknown whether it is possible to generalize the analysis in \citet{cai2020provably} to  handle linear MDPs. 
 % While our method is very close to that of  \citet{cai2020provably} (policy optimization, with bonuses), our analyses diverts from theirs to avoid this issue, while we, just like them, also use LSPE to evaluate policies). 
\citet{agarwal2020pc,zanette2021cautiously} derive the first line of policy optimization results for RL in linear MDPs without any reachability (or coverage) style assumption. 
Compared to \citet{agarwal2020pc,zanette2021cautiously}, this paper considers the same setting but designs a simpler algorithm with cleaner analysis and sharper sample complexity guarantee. Nevertheless, we remark that in certain model misspecification setting, the algorithms in \citet{agarwal2020pc,zanette2021cautiously} can potentially achieve stronger guarantees. Since this paper focuses on the well-specified setting (that is, the environment is perfectly modeled by a linear MDP), we refer interested readers to \citet{agarwal2020pc} for more details. 
Finally, there have been a long line of works \citep[e.g.,][, etc]{agarwal2021theory,bhandari2019global,liu2019neural,neu2017unified,abbasi2019politex} that study policy optimization under reachability (or coverage) assumptions, which largely reduce the difficulty of learning a good policy. 
Throughout this paper we do not make any such assumption  and  directly tackle the exploration challenge.
 
 \paragraph{Linear MDPs.}
 
\citet{jin2020provably} proposed a computationally efficient algorithm (LSVI-UCB) with  
$\tilde{\cO}(d^3/\epsilon^2)$ sample complexity. 
Later on, \citet{zanette2020learning} utilized the idea of global optimism to obtain the optimal  sample complexity $\tilde{\Theta}(d^2/\epsilon^2)$  at the cost of sacrificing  computational efficiency.
Recently, \citet{he2022nearly,agarwal2022vo,wagenmaker2022reward} design new computationally efficient algorithms that can achieve  $\tilde{\cO}(d^2/\epsilon^2+d^{\ge 4}/\epsilon)$ sample complexity. 
Compared to the above works, the sample complexity of \oppo~is not strictly worse than that of any known computationally efficient algorithm. In fact, it is the only computationally efficient one to achieve the optimal  dimension dependence.
Nonetheless, for learning a near-optimal policy with a  vanishing suboptimality $\epsilon$, the current sample complexity of \oppo~is loose by a factor of $\epsilon^{-1}$.
 
 

 
 
 


==> legacy/linear.tex <==
%!TEX root =  main.tex
\section{Optimistic Natural Policy Gradient}

In this section, we present the algorithm \oppo~(Optimistic Natural Policy Gradient) and its theoretical guarantees.

\subsection{Algorithm} The pseudocode of \oppo~is provided in Algorithm \ref{alg:oppo}.
At a high level, the algorithm consists of the following three key modules. 
\begin{itemize}
    \item \textbf{Periodic on-policy data collection} (Line \ref{line:sample-0}-\ref{line:sample-1}): Similar to the standard PPO algorithm,  \oppo~discards all the old data, and  
     executes the \emph{current} policy $\pi^k$ to collect a batch of fresh data $\cD^k$ after every $m$ steps of policy update. These  data will later be  used to evaluate and improve the policies in the next $m$ steps. 
    Noticeably, this \emph{on-policy} data mechanism is very different from most existing works in theoretical RL, where they either need to keep the historical data or have to rerun historical policies to refresh the dataset for the technical purpose of elliptical potential arguments in proofs. 
    In comparison, \oppo~only uses the fresh data collected by the current (or very recent) policy, which resembles the practical policy optimization algorithms (PPO, TRPO, etc) widely used in empirical RL.
    \item \textbf{Optimistic policy evaluation}  (Line \ref{line:pe}): Given the above collected dataset $\cD^k$, we can estimate the value functions of the current policy $\pi^k$ by invoking Algorithm \ref{alg:lspe} \lspe~(optimistic least-square policy evaluation). At a high level, \lspe~computes an  upper bound $\overline{Q}$ for $Q^{\pi}$ by using the Bellman equation under policy $\pi$ backwards from step $H$ to step $1$ while adding a bonus to compensate the uncertainty of parameter estimation.
    Specifically, the step of ridge regression (Line \ref{line:ridge}) utilizes the linear completeness property of linear MDPs in computing $\overline{Q}_h$ from $\overline{V}_{h+1}$, which states that for any function $\oV_{h+1}:\cS\rightarrow\R$, there exists $\otheta_h\in\R^d$ so that
    $\langle \phi_h(s,a),\otheta_h\rangle = R_h(s,a)+\E_{s'\sim\P_h(\cdot\mid s,a)}[\oV_{h+1}(s')]$ for all $(s,a)\in\cS\times\cA$.
    And in Line \ref{line:bonus}, we add an elliptical bonus $b_h(s,a)$ to compensate the error between our estimate $\hat\theta_h$ and the groundtruth $\otheta_h$ so that we can  guarantee $\oQ_h\ge Q^\pi_h$  with high probability by backward induction on $h$.
\begin{equation}
\label{eq:ridge}
\begin{aligned}
\hat \theta_h &=  \argmin_{\theta}
\hspace{-6mm}\sum_{(s_h,a_h,r_h,s_{h+1})\in\cD_h} \bigg(\phi_h(s_h,a_h)\trans\theta \\
&\qquad\qquad -  r_h - \oV_{h+1}(s_{h+1}) \bigg)^2 + \lambda \|\theta\|_2^2.
\end{aligned}
\end{equation}
    \item \textbf{Policy update} (Line \ref{line:pu}): Given the optimistic value estimates $\{\oQ^k_h\}_{h\in[H]}$ of $\pi^k$, \oppo~performs one-step mirror ascent from $\pi_h^k(\cdot \mid s)$ with gradient $\oQ^k_h(s,\cdot)$  to obtain
    $\pi_h^{k+1}(\cdot \mid s)$ at each $(h,s)$. We remark that this step can be implemented in a computationally efficient way, because by the update rule of mirror ascent $\pi^{k}_h(\cdot\mid s)\propto \exp(\eta\sum_{t=1}^{k-1} \oQ_h^t(s,\cdot))$, we only need to store $\{\{\oQ_h^t\}_{h\in[H]}\}_{t\in[K]}$, from which any $\pi^{k}_h(\cdot\mid s)$ can be computed on the fly.
\end{itemize}

\begin{algorithm}[t]
\caption{\oppo}
\label{alg:oppo}
\begin{algorithmic}[1]
\STATE \textbf{input}: 
number of iterations $K$, period of collecting fresh data  $m$, data batch size $N$, learning rate $\eta$, $\lspe$ parameters $\lambda$ and $\alpha$
\STATE \textbf{initialize:} for all $(h,s)\in[H]\times\cS$\\
~~~~~~~~~~~~~set $\pi^1_h(\cdot\mid s)={\rm Uniform}(\mathcal{A})$ 
\FOR{$k=1,\ldots,K$}
\IF{$k\equiv 1 (\mbox{mod } m)$} \label{line:sample-0}
\STATE 
$\cD^k\setto$ $\{N$ fresh trajectories $\stackrel{\text{i.i.d.}}{\sim}\pi^k\}$
\ELSE 
\STATE $\cD^k  \setto \cD^{k-1}$ 
\ENDIF \label{line:sample-1}
\STATE  
$\{\oQ^k_h\}_{h\in[H]} \leftarrow\lspe(\pi^k, \cD^k,\lambda,\alpha)$
\label{line:pe}
\STATE for all $(h,s)\in[H]\times\cS$\\
~~~~~update  $\pi^{k+1}_h(\cdot\mid s) \propto \pi^{k}_h(\cdot\mid s) \cdot \exp( \eta \cdot \oQ_h^k(s,\cdot))$ 
\label{line:pu}
\ENDFOR
\STATE \textbf{output}: $\piout$ that is sampled u.a.r. from $\{\pi^k\}_{k\in[K]}$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
\caption{$\lspe(\pi, \cD,\lambda,\alpha)$}
\label{alg:lspe}
\begin{algorithmic}[1]
\STATE split $\cD$ evenly into $H$ disjoint subsets $\cD_1,\ldots,\cD_H$
\label{line:split}
\STATE  set $\oV_{H+1}(s)\setto 0$ for all $s\in\cS$
\FOR{$h=H:1$}
\STATE perform ridge regression according to Equation \eqref{eq:ridge}
\label{line:ridge}
\STATE compute covariance matrix\\ ~\quad$\Sigma_h = \sum_{(s_h,a_h)\in\cD_h} \phi_h(s_h,a_h) \phi_h(s_h,a_h)\trans$\\ and define \vspace{-3mm}
\begin{equation*}\vspace{-1mm}
\begin{cases}
    \oQ_h(s,a)= {\rm Truncate}_{[0,H-h+1]}\big( \\
    \qquad\qquad \langle \hat \theta_h, \phi_h(s,a)\rangle + b_h(s,a)\big) \\
    \oV_h(s)= \E_{a\sim \pi_h(\cdot\mid s)}\left[ \oQ_h(s,a)\right]\vspace{-2mm}
    \end{cases}
\end{equation*}
  with bonus function\\ $~\qquad b_h(s,a):=\alpha\times \|\phi_h(s,a)\|_{(\Sigma_h +\lambda \I_{d\times d})^{-1} }$\label{line:bonus}
\ENDFOR
\STATE \textbf{output}  $\{\oQ_h\}_{h=1}^H$
\end{algorithmic}
\end{algorithm}

\subsection{Theoretical guarantee}
We have the following theoretical guarantees for \oppo, which we prove in Section~\ref{sec:proof-sketch}.

\begin{theorem}\label{thm:main}
In Algorithm \ref{alg:oppo}, if we choose
\begin{align*}
&K =\Theta\left(\frac{H^4\log|\cA|}{\epsilon^2}\right),\quad
N=\Theta\left(\frac{d^2 H^3 \log^2(Kd)}{\epsilon^2}\right), \\
&\eta =\Theta\left(\frac{\epsilon}{H^3}\right),\quad
\quad m\le \Theta\left(\frac{H}{\epsilon}\right),\\
& \lambda =1, \qquad
\alpha =\Theta\left(H\sqrt{d\log(KN)}\right),
\end{align*}
 then with probability at least $1/2$, $\piout$  is $\cO(\epsilon)$-optimal. 
\end{theorem}
Below we emphasize two special choices of $m$ (the period of sampling fresh data) in Theorem \ref{thm:main}: 

\begin{itemize}
    \item When choosing $m=1$, \oppo~is purely on-policy as it only uses data sampled from the current policy to perform policy optimization. In this case, the total sample complexity is 
    $$
    \frac{KN}{m}= \tilde{\Theta}\left( \frac{d^2 H^7}{\epsilon^4}\right).
    $$
    \item When choosing $m=[1/(H^2\eta)]$, we obtain sample complexity 
     $$
    \frac{KN}{m}= \tilde{\Theta}\left( \frac{d^2 H^6}{\epsilon^3}\right),
    $$
    which improves  over the best existing policy optimization results \citep{zanette2021cautiously} by a factor of $d$.
\end{itemize}

% An immediate consequence of Theorem \ref{thm:main} is that $(KN/m)=\tilde{\cO}(\poly(H)d^2/\epsilon^3)$ episodes suffice for learning an $\epsilon$-optimal policy, which improves  over the SOTA policy optimization results \citep{zanette2021cautiously} by a factor of $d$.
% Moreover, to our knowledge, \oppo~is the first computationally efficient algorithm to achieve the optimal dimension dependence ($d^2$) in the regime where  $\epsilon$ is of order constant,  e.g., $\epsilon=10^{-3}$. 
Notably, both above results have the optimal quadratic dimension dependence, which are the first to achieve so among computationally efficient algorithms. 
The key reason behind this improvement is that \oppo~periodically collects on-policy fresh data, which
removes some undesired correlation (and union bound) that commonly appears in previous works.
As a result, \oppo~uses a bonus function that is smaller by a factor of $\sqrt{d}$ than previous works \citep[e.g.,][]{jin2020provably}. 
We refer interested readers to Section \ref{sec:proof-sketch} (in particular, Lemma \ref{lem:opt}) for more details on how we achieve this improvement.




Given the improved rate \oppo~achieves in the linear setting, it is natural to ask how it compares to previous works on policy optimization when being specialized to the basic tabular setting.
By simple observation, one can see that Algorithm \ref{alg:oppo} remains the same while Algorithm \ref{alg:lspe} roughly degenerates to Algorithm \ref{alg:tabpe} which  evaluates policy $\pi$ using the empirical model estimated from $\cD$ and additionally adds standard UCB bonus to compensate the uncertainty in model estimation. Formally, we have the following guarantee for RL of  tabular MDPs with \oppo.

\allowdisplaybreaks
\begin{theorem}[tabular MDPs]\label{thm:tabular}
In Algorithm \ref{alg:oppo}, if we replace $\lspe$ with Algorithm \ref{alg:tabpe} and  choose
\begin{align*}
&K =\Theta\left(\frac{H^4\log|\cA|}{\epsilon^2}\right),\\
&N=\Theta\left(\frac{|\cS||\cA| H^3  \log^2(K|\cS||\cA|)}{\epsilon^2}\right), \\
&\eta =\Theta\left(\frac{\epsilon}{H^3}\right),\quad
\quad m\le \Theta\left(\frac{H}{\epsilon}\right),\\
& 
\alpha =\Theta\left(H\sqrt{\log(KHSA)}\right),
\end{align*}
 then with probability at least $1/2$, $\piout$  is $\cO(\epsilon)$-optimal. 
\end{theorem}
The proof of  Theorem \ref{thm:tabular} closely resembles that of Theorem \ref{thm:main} and we postpone it to Appendix \ref{app:tab}.
 When choosing $m=[1/(H^2\eta)]$, Theorem \ref{thm:tabular} implies that \oppo~learns an $\epsilon$-optimal policy within $(KN/m)=\tilde{\cO}(H^6|\cS||\cA|/\epsilon^3)$ episodes  for any tabular MDP. Compared to the SOTA results $\tilde{\cO}(H^4|\cS|^2|\cA|/\epsilon^2)$ achieved by policy optimization algorithms \citep{shani2020optimistic}, Theorem \ref{thm:tabular} has better $|\cS|$-dependence but worse  dependence on $\epsilon$ and $H$.
 To our knowledge, it remains open how to achieve the optimal rate 
 $\tilde{\Theta}(H^3|\cS||\cA|/\epsilon^2)$ by policy optimization algorithms.
 
Finally, note that for simplicity we stated both our main results for a fixed, constant failure probability. 
However, the result is easy to extend to the case when the failure probability is some arbitrary value of $\delta\in (0,1)$ at the  expense of increasing the sample complexity by a factor of $\log(1/\delta)$.





\begin{algorithm}[t]
\caption{$\pe(\pi, \cD,\alpha)$}
\label{alg:tabpe}
\begin{algorithmic}[1]
\STATE split $\cD$ evenly into $H$ disjoint subsets $\cD_1,\ldots,\cD_H$
\STATE compute empirical estimate $(\hat\P_h,\hat R_h)$ of the transition and reward at step $h$ by using $\cD_h$
\STATE  set $\oV_{H+1}(s)\setto 0$ for all $s\in\cS$
\FOR{$h=H:1$}
\STATE for all $(h,s,a)\in[H]\times\cS\times\cA$, compute \\
$~\quad J_h(s,a)\setto\sum_{(s_h,a_h)\in\cD_h}\mathbf{1}((s_h,a_h)=(s,a))$\\
and define\vspace{-2mm}
\begin{equation*}\vspace{-3mm}
\begin{cases}
    &\oQ_h(s,a)= \min\big\{H-h+1,~\\
    &\quad\E_{s'\sim\hat\P_h (s,a)}[ \oV_{h+1}(s')]+\hat R_h(s,a)+ b_h(s,a)\big\}  \\
    &\oV_h(s)= \E_{a\sim \pi_h(\cdot\mid s)}\left[ \oQ_h(s,a)\right]
    \end{cases}
\end{equation*}
  with bonus function\\ \quad\quad $b_h(s,a)=\alpha({J_h(s,a)+1})^{-1/2}$
\ENDFOR
\STATE \textbf{output}  $\{\oQ_h\}_{h=1}^H$
\end{algorithmic}
\end{algorithm}

==> legacy/notations.tex <==
%!TEX root =  main.tex
%\usepackage{fullpage}

\usepackage{mathtools}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2023} with \usepackage[nohyperref]{icml2023} above.
\usepackage{hyperref}


% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}


\usepackage{natbib}
\usepackage{color}
\usepackage{amsmath}
\usepackage{bm}
\usepackage{amsthm}
\usepackage{amsfonts}

%\usepackage{algorithm}
%\usepackage[noend]{algorithmic}


\newcommand{\piout}{\pi^{\rm out}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\B}{\mathbb{B}}

\newcommand{\w}{\mathbf{w}}
\newcommand{\btheta}{\bm{\theta}}

\newcommand{\cD}{\mathcal{D}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cM}{\mathcal{M}}

\newcommand{\up}[1]{{ #1}}
\renewcommand{\th}{^{\rm th}}
\newcommand{\argmax}{{\rm argmax}}
\newcommand{\argmin}{{\rm argmin}}
\newcommand{\alg}{\textsc{Routine}}
\newcommand{\reg}{\textrm{Regret}}
\newcommand{\poly}{{\mathrm{poly}}}
\newcommand{\ellip}{\textrm{Estimate}}
\newcommand{\trans}{^{\rm T}}
\newcommand{\Cov}{{\rm Cov}}
\newcommand{\setto}{\leftarrow}
\newcommand{\oV}{\overline{V}}
\newcommand{\oQ}{\overline{Q}}
\newcommand{\otheta}{\overline{\theta}}


\newtheorem{condition}{Condition}
\newtheorem{theorem}{Theorem}
\newtheorem{observation}{Observation}
\newtheorem{remark}{Remark}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}

% \newcommand{\lspe}{\textsf{LSPE}$-$\textsc{bonus}}
\newcommand{\lspe}{\textsf{Optimistic LSPE}}
\newcommand{\pe}{\textsf{Optimistic tabular PE}}
\newcommand{\oppo}{\textsf{Optimistic NPG}}



==> legacy/old_notes.tex <==

\section{Pipeline for Analyzing Policy Optimization Algorithms}

Below we provide a unified view for the proofs in  previous policy optimization papers \cite{shani2020optimistic, cai2020provably}, in a high-level and abstract way.

\subsection{Meta algorithm}

\begin{algorithm}\label{alg:1}
\caption{Optimistic Policy Optimization}
\begin{algorithmic}
\STATE initialize $\pi^1_h(\cdot\mid s)={\rm Uniform}(\mathcal{A})$ for all $h,s$
\FOR{$k=1,\ldots,K$}
\STATE execute $\pi^k$ to collect $\tau^k=(s_1^k,a_1^k,r_1^k,\ldots,s_H^k,a_H^k,r_H^k)$
\STATE compute an estimate $\up{Q}_h^k(s,a)$ for $Q_h^{\pi^k}(s,a)$ using the collected data
\STATE update  $\pi^{k+1}\longleftarrow \alg(\{\up{Q}^t\}_{t=1}^k)$
\ENDFOR
\end{algorithmic}
\end{algorithm}


\subsection{Meta theorem}


\begin{condition}\label{cond:1}
The value estimator $\{\up{Q}^k\}_{k=1}^K$ and \alg\ in Algorithm \ref{alg:1} satisfy 
\begin{enumerate}
    \item \textbf{No-regret}:  $\sum_{k=1}^K\langle \mu - \pi^k_h(\cdot\mid s), \up{Q}^k_h(s,\cdot) \rangle  \le \reg(K) $ for any $s,h$ and $\mu\in\Delta_A$.
    \item \textbf{Optimistic Bellman-consistency}: $\up{Q}_h^k(s,a) \ge [\mathcal{T}^{\pi^k}\up{Q}_{h+1}^k](s,a)$ for any $(s,a,h)$.
    \item \textbf{Pigeon-hole}: $\sum_{k=1}^K \left(V_1^k(s_1) - V_1^{\pi^k}(s_1) \right)\le \ellip(K)$ where $V_h^k(s)=\langle \pi_h^k(\cdot\mid s), Q_h^k(s,\cdot)\rangle$.
\end{enumerate}
\end{condition}

\begin{theorem}
Suppose Condition \ref{cond:1} holds, then
$$
\sum_{k=1}^K \left( V^\star_1(s_1) - V_1^{\pi^k}(s_1) \right)\le \ellip(K) + \reg(K).
$$
\end{theorem}
\begin{proof}
We use $V^k$ as an intermediate quantity for controlling the regret:
$$
\sum_{k=1}^K \left( V^\star_1(s_1) - V_1^{\pi^k}(s_1) \right) 
= \sum_{k=1}^K \left( V^\star_1(s_1) - V_1^{k}(s_1) \right)  + \sum_{k=1}^K \left( V^k_1(s_1) - V_1^{\pi^k}(s_1) \right) 
$$

The second quantity is upper bounded by $\ellip(K) $ by the \textbf{pigeon-hole} condition.  

For the first quantity, we can use the performance difference lemma (e.g., Lemma 3.2 in \cite{cai2020provably}) together with the \textbf{optimistic Bellman-consistency} condition to get 
$$
\sum_{k=1}^K \left( V^\star_1(s_1) - V_1^{k}(s_1) \right)  \le \sum_{h=1}^H \E_{s_h\sim {\pi^\star}} \left[ \sum_{k=1}^K\langle \pi_h^\star(\cdot \mid s_h) - \pi^k_h(\cdot\mid s), \up{Q}^k_h(s,\cdot) \rangle \right],
$$
which is upper bounded by $\reg(K)$ by the \textbf{no-regret} condition.
\end{proof}


\subsection{Discussions on Condition \ref{cond:1}}

So the question is how to guarantee Condition \ref{cond:1}.

\paragraph{1. No-regret} This can be easily achieved by  no-regret online learning algorithms, e.g., mirror descent 
$$\pi^{k+1}_h(a\mid s) \propto \exp\left( \eta \sum_{t=1}^k \up{Q}_h^k(s,a) \right).$$


In \cite{cai2020provably}, they adopt the following design for $Q^k$:
$$
\begin{cases}
Q_h^k(s,a) = \text{Truncate}_{[0,H-h+1]} \left\{[\widehat{\P}_h^k V_{h+1}^k](s,a) + r_h(s,a)+b_h^k(s,a)\right\}, \\
V_h^k(s) = \langle \pi_h^k(\cdot \mid s), Q_h^k(s,\cdot) \rangle,
\end{cases}
$$
where $\P_h^k$ is the empirical estimate of the transition and $b_h^k(s,a)$ is certain bonus function (e.g., for example $\sim 1/\sqrt{n_h^k(s,a)}$ in the tabular setting and $\sim\|\phi_{h}(s,a)\|_{\Sigma_h^k}$ in the linear setting). 


\paragraph{2. Optimistic Bellman-consistency} This is true if we have 
$$
\left \langle (\P_h-\widehat{\P}_h^k)(s,a), V_{h+1}^k \right\rangle_{\mathcal{S}}  \le b_h^k(s,a).
$$


\paragraph{3. Pigeon-hole} This is true if 
$$
\left \langle (\widehat{\P}_h^k-\P_h)(s,a), V_{h+1}^k \right\rangle_{\mathcal{S}}   \le b_h^k(s,a),
$$
because by iteratively utilizing the above inequality, we have 
$$
\sum_{k=1}^K \left(V_1^k(s_1) - V_1^{\pi^k}(s_1) \right) = \mathcal{O}(1)\times \sum_{h=1}^H \sum_{k=1}^k \E_{(s_h,a_h)\sim {\pi^k}}\left[ b_h^k(s_h,a_h)\right],
$$
which is further controlled by the pigeon-hole or the elliptical potential arguments.

\subsection{Key challenge}
How to guarantee 
$$
\left|\left \langle (\widehat{\P}_h^k-\P_h)(s,a), V_{h+1}^k \right\rangle_{\mathcal{S}}  \right| \le b_h^k(s,a).
$$


\section{Alternative Algorithm Designs}


\subsection{On-policy policy optimization}

\begin{algorithm}[H]
\caption{Optimistic Policy Optimization with Fresh Data }
\label{alg:new}
\begin{algorithmic}
\STATE initialize $\pi^1_h(\cdot\mid s)={\rm Uniform}(\mathcal{A})$ for all $h,s$
\FOR{$k=1,\ldots,K$}
\STATE run {\color{red} $\pi^k$} to collect $H$ batches of trajectories  $\{\cD^k_h\}_{h=1}^H$,  each of which is of size $N$ 
\STATE compute  $\up{Q}^k \leftarrow \lsvi (\pi^k, \{\cD^k_h\}_{h=1}^H)$
\STATE update  $\pi^{k+1}_h(a\mid s) \propto \pi^{k}_h(a\mid s) \cdot \exp\left( \eta \cdot \up{Q}_h^k(s,a) \right)$
\ENDFOR
\STATE output $\piout$ that is sampled u.a.r. from $\{\pi^k\}_{k=1}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{$\lsvi (\pi, \{\cD_h\}_{h=1}^H)$}
\label{alg:lsvi}
\begin{algorithmic}
\STATE Initialize $V_{H+1}(s)=0$ for all $s$
\FOR{$h=H:1$}
\STATE compute covariance matrix $\Sigma_h = \sum_{(s_h,a_h)\in\cD_h} \phi_h(s_h,a_h) \phi_h(s_h,a_h)\trans$
\STATE perform ridge regression $\hat \theta_h = (\Sigma_h +\lambda \I_{d\times d})^{-1} \sum_{(s_h,a_h,r_h,s_{h+1})\in\cD_h} \phi_h(s_h,a_h) \left(r_h + V_{h+1}(s_{h+1}) \right)$
\STATE compute elliptical bonus $b_h(s,a)=\tilde{\cO}(\sqrt{d})\cdot  \|\phi_h(s,a)\|_{(\Sigma_h +\lambda \I_{d\times d})^{-1} }$
\STATE  $Q_h(s,a)= {\rm Truncate}_{[0,H-h+1]}\left( \langle \hat \theta_h, \phi_h(s,a)\rangle + b_h(s,a)\right) $
\STATE $V_h(s)= \E_{a\sim \pi_h(s)}[Q_h(s,a)]$
\ENDFOR
\STATE return functions $\{Q_h\}_{h=1}^H$
\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{thm:main}
In Algorithm \ref{alg:new}, if we choose $N=\tilde{\mathcal{O}}(\poly(H)d^2/\epsilon^2)$,  $K=\tilde{\mathcal{O}}(\poly(H)/\epsilon^2)$ and $\eta=\tilde{\mathcal{O}}(1/(H\sqrt{K}))$, then with probability at least $1/2$, $\piout$  is $\epsilon$-optimal. 
\end{theorem}




\subsection{Off-policy policy iteration}


\paragraph{Optimistic policy iteration:} easy to cover the policy class and should give $\sqrt{d^3K}$-regret guarantee?

\begin{algorithm}[H]
\caption{Optimistic Policy Iteration}
\begin{algorithmic}
\STATE initialize $\pi^1_h(\cdot\mid s)={\rm Uniform}(\mathcal{A})$ for all $h,s$
\FOR{$k=1,\ldots,K$}
\STATE execute $\pi^k$ to collect $\tau^k=(s_1^k,a_1^k,r_1^k,\ldots,s_H^k,a_H^k,r_H^k)$
\STATE compute an optimistic estimate $\up{Q}_h^k(s,a)$ for $Q_h^{\pi^k}(s,a)$ using the collected data
\STATE update  $\pi^{k+1}$ to be the greedy policy w.r.t. $\up{Q}_h^k(s,a)$
\ENDFOR
\end{algorithmic}
\end{algorithm}





\subsection{Adversarial setting}


\paragraph{Two-stage algorithms:}
If our goal is only about to handle adversarial reward, then maybe we could try some hybrid algorithms e.g.,  reward-free learning \cite{wang2020reward} + policy gradient-style algorithms as suggested by Gellért. 






\bibliography{ref}
\bibliographystyle{alpha}


\appendix 

\section{Supporting Lemmas}

\begin{lemma}
 [generalized policy-difference lemma, e.g., Lemma 1 in  \cite{shani2020optimistic}]\label{lem:pi-diff}
 For any policy $\pi$, 
 \begin{equation}
 \begin{aligned}
      V_1^\pi(s_1) - V_1^k (s_1)  
     = & \sum_{h=1}^H \E_{s_h\sim\pi} \left[\langle \pi_h(\cdot\mid s_h)- \pi^k_h(\cdot\mid s_h),  Q^k_h(s_h,\cdot)\rangle  \right] \\
     &- 
     \sum_{h=1}^H \E_{(s_h,a_h)\sim\pi} \left[Q_h^k(s_h,a_h) - r_h(s_h,a_h)- [\P_h V_{h+1}^k](s_h,a_h) \right].
     \end{aligned}
 \end{equation}
\end{lemma}

\begin{proposition}[on-policy uncertainty shrinkage] \label{prop:optimism-upper-bound}
Given any policy $\pi$ and $\lambda \ge R_\phi$, suppose we execute $\pi$ for $N$ episodes to collect trajectories $\{\{(s_h^n,a_h^n)\}_{h=1}^H\}_{n=1}^N$. 
Denote bonus function $\beta_h^n(s,a) := \|\phi_h(s,a)\|_{(\Sigma_h^n)^{-1}}$ where $\Sigma_h^n=\sum_{i=1}^{n-1} \phi_h(s_h^i,a_h^i) \phi_h\trans(s_h^i,a_h^i) + \lambda^2  \I_{d\times d}$. 
Then with  probability at least $1-\delta$: we have that for all $h\in[H]$
$$
\E_{\pi}[\beta_h^N(s_h,a_h)] 
= \cO\left(\sqrt{\frac{d\log(NR_\phi /\lambda)}{N} }\right)+ \cO\left(\frac{R_\phi}{\lambda}\sqrt{\frac{\log(H/\delta)}{N}}\right).
$$
\end{proposition}
\begin{proof}[Proof of Proposition \ref{prop:optimism-upper-bound}]
Without loss of generality, we consider a fixed $h\in[H]$ and denote $\phi^i_h :=\phi_h(s_h^i,a_h^i)$.  
By Azuma-Hoeffding inequality, we have  with probability at least $1-\delta$: 
\begin{equation}
\begin{aligned}
  \sum_{n=1}^N \E_{\pi}[\beta_h^n(s_h,a_h)]
& \le \sum_{n=1}^N \beta_h^n(s_h^n,a_h^n) + \cO\left(\frac{R_\phi}{\lambda}\sqrt{N\log(1/\delta)}\right)\\
&  =    \sum_{n=1}^N 
\|\phi^n_h\|_{(\Sigma_h^n)^{-1}} + \cO\left(\frac{R_\phi}{\lambda}\sqrt{N\log(1/\delta)}\right) \\
& = \cO\left(\sqrt{dN\log(NR_\phi /\lambda) }\right)+ \cO\left(\frac{R_\phi}{\lambda}\sqrt{N\log(1/\delta)}\right).
\end{aligned}
\end{equation}
Notice that $\beta_h^n$ is monotonically decreasing with respect to $n$, so we have 
$$
\E_{\pi}[\beta_h^N(s_h,a_h)] \le 
\frac{1}{N}\sum_{n=1}^N \E_{\pi}[\beta_h^n(s_h,a_h)]
 = \cO\left(\sqrt{\frac{d\log(NR_\phi /\lambda)}{N} }\right)+ \cO\left(\frac{R_\phi}{\lambda}\sqrt{\frac{\log(1/\delta)}{N}}\right).
$$
By taking a union bound for all $h\in[H]$, we completes the proof.
\end{proof}

\begin{lemma}[Concentration]\label{lem:concen}
 Suppose we sample $\cD:=\{(s_h^i,a_h^i,s_{h+1}^i)\}_{i=1}^n$ from an arbitrary policy. Let 
 \begin{itemize}
     \item $V_{h+1}:\cS\rightarrow [0,H]$ be a function independent of $\cD$,
     \item $\theta\in B_{H\sqrt{d}}(0)$ s.t. 
     $\langle \phi_h(s,a), \theta\rangle = r_h(s,a) + [\P_h V_{h+1}](s,a)$
     for all $(s,a)$,
     \item $\hat\theta = (\sum_{i=1}^n \phi^i{\phi^i}\trans + \lambda^2 \I_{d\times d})^{-1}\sum_{i=1}^m \phi^i [r^i+V_{h+1}^i]$ where $\phi_i:=\phi_h(s_h^i,a_h^i)$, $r^i:=r_h(s_h^i,a_h^i)$, and $V^i:=V_h(s_{h+1}^i)$.
 \end{itemize} 
 Then with probability $1-\delta$, we have that for any $(s,a)\in\cS\times\cA$:
 $$
 \left|\langle \theta-\hat\theta, \phi_h(s,a)\rangle \right|=  \left\| \phi_h(s,a)\right\|_{\left(\Cov+ \lambda^2 \I_{d\times d}\right)^{-1}} \times \cO\left(\sqrt{d\log(d/\delta)} +\lambda R_\theta\right). 
 $$
\end{lemma}
\begin{proof}
To simplify notations, denote $\Cov=\sum_{i=1}^n \phi^i{\phi^i}\trans$.  
\begin{equation}
    \begin{aligned}
    &\left|\langle\phi_h(s,a),  \theta-\hat\theta \rangle \right| \\
    = &\left|\left\langle\phi_h(s,a),   \left(\Cov + \lambda^2 \I_{d\times d}\right)^{-1}\left( \sum_i \phi^i [r^i+V^i] - \left(\Cov + \lambda^2 \I_{d\times d}\right)\theta \right) \right\rangle\right| \\
    \le & \left\| \phi_h(s,a)\right\|_{\left(\Cov+ \lambda^2 \I_{d\times d}\right)^{-1}} \times \left( \left\| \sum_i \phi^i [r^i+V^i-{\phi^i}\trans\theta]  \right\|_{\left(\Cov+ \lambda^2 \I_{d\times d}\right)^{-1}} + \lambda \left\|\theta \right\|_2
    \right) \\
    \le &  \left\| \phi_h(s,a)\right\|_{\left(\Cov+ \lambda^2 \I_{d\times d}\right)^{-1}} \times \left( \left\| \sum_i \phi^i \left[r^i+V^i-\E[r^i+V^i\mid s_h^i,a_h^i]\right]  \right\|_{\left(\Cov+ \lambda^2 \I_{d\times d}\right)^{-1}} + \lambda R_\theta
    \right) \\
    = &   \left\| \phi_h(s,a)\right\|_{\left(\Cov+ \lambda^2 \I_{d\times d}\right)^{-1}} \times \cO\left(\sqrt{d\log(d/\delta)} +\lambda R_\theta\right),
    \end{aligned}
\end{equation}
where the last relation holds with probability at least $1-\delta$ by standard vector concentration. 
\end{proof}

\begin{lemma}[MD regret]\label{lem:md}
Suppose $\eta\le 1/H$. Then for all $(h,s,K)$ and $\mu\in\Delta_A$
$$
\sum_{k=1}^K\langle \mu - \pi^k_h(\cdot\mid s), \up{Q}^k_h(s,\cdot) \rangle = \cO\left( \frac{\log A}{\eta} + \eta K H^2 \right).
$$
\end{lemma}

\begin{lemma}[Optimism]\label{lem:optimism} With probability at least $1-\delta$, for all $(h,s,k)\in[H]\times\cS\times[K]$:
$$
\begin{cases}
r_h(s_h,a_h)+ [\P_h V_{h+1}^k](s_h,a_h)  \le 
Q_h^{k}(s_h,a_h)\\
Q_h^{k}(s_h,a_h) \le 
r_h(s_h,a_h)+ [\P_h V_{h+1}^k](s_h,a_h) + 2 b_h^k(s_h,a_h),
\end{cases}
$$
where $b_h^k(s,a):= \left\| \phi_h(s,a)\right\|_{\left(\Cov+ \lambda^2 \I_{d\times d}\right)^{-1}} \times \cO\left(\sqrt{d\log(d/\delta)} +\lambda R_\theta\right)$.
\end{lemma}

\subsection{Proof of Theorem \ref{thm:main}}
\begin{equation}
    \begin{aligned}
    {\rm Regret}(T)= & N \sum_{k=1}^K \left( V^\star_1(s_1) - V_1^{\pi^k}(s_1) \right) \\
= & N \sum_{k=1}^K \left( V^\star_1(s_1) - V_1^{k}(s_1) \right)  + N\sum_{k=1}^K \left( V^k_1(s_1) - V_1^{\pi^k}(s_1) \right) \\ (\text{Lemma \ref{lem:pi-diff} \& \ref{lem:optimism}}) \le & 
N\sum_{h=1}^H \E_{s_h\sim {\pi^\star}} \left[ \sum_{k=1}^K\langle \pi_h^\star(\cdot \mid s_h) - \pi^k_h(\cdot\mid s), \up{Q}^k_h(s,\cdot) \rangle \right] \\
(\text{Lemma  \ref{lem:optimism}}) \quad  &+
2N\sum_{k=1}^K \sum_{h=1}^H \E_{\pi^k}[b_h^k(s_h,a_h)]
\\
(\text{Lemma \ref{lem:md} \& Proposition \ref{prop:optimism-upper-bound}})\le & NH \times \cO\left( \frac{\log A}{\eta} + \eta K H^2 +HK\sqrt{d\log(d/\delta)}  \times \sqrt{\frac{dH\log N}{N}} \right) \\
\le & \log^2(ANd/\delta) NH^2 \times 
\cO\left( \frac{1}{\eta} + \eta K H +dK\sqrt{\frac{H}{N}} \right) 
    \end{aligned}
\end{equation}
where the second inequality  uses the fact that $R_\theta \le H\sqrt{d}$, $R_\phi=\lambda=1$.

By picking $\eta=\sqrt{1/(KH)}$, we have 
$$
{\rm Regret}(T) 
\le  \log^2(ANd/\delta) H^{2.5} \times 
\cO\left( \sqrt{K}N +dK\sqrt{N} \right).
$$
 Recall that the total number of episodes is $T=KN$, so we can pick $K=\sqrt{T}/d$ and $N=\sqrt{T}\times d$, which gives 
 $$
 {\rm Regret}(T)  \le 
\cO\left(   H^{2.5}\cdot  \sqrt{d}\cdot 
  T^{3/4} \cdot\log^2(TA/\delta)\right).
 $$

==> legacy/pre-icml-notes.tex <==
\section{Proof of Theorem \ref{thm:main}}

Let $T:=KNH/m$ denote the total number of episodes we have sampled from the linear MDP.  
\begin{equation}
    \begin{aligned}
    {\rm Regret}(K)= &  \sum_{k=1}^K \left( V^\star_1(s_1) - V_1^{\pi^k}(s_1) \right)  \\
= &  \sum_{k=1}^K \left( V^\star_1(s_1) - V_1^{k}(s_1) \right)   + \sum_{k=1}^K \left( V^k_1(s_1) - V_1^{\pi^k}(s_1) \right)  \\ (\text{Lemma \ref{lem:pi-diff} \& \ref{lem:optimism}}) \le & \sum_{h=1}^H \E_{s_h\sim {\pi^\star}} \left[ \sum_{k=1}^K\left\langle \pi_h^\star(\cdot \mid s_h) - \pi^k_h(\cdot\mid s), \up{Q}^k_h(s,\cdot) \right\rangle \right]  \\
(\text{Lemma  \ref{lem:optimism}}) \quad  &+
2\sum_{k=1}^K \sum_{h=1}^H \E_{\pi^k}[b_h^k(s_h,a_h)]  
\\
(\text{Lemma \ref{lem:md} \& Corollary \ref{cor:bonus}})\le & \cO\left( \frac{\log A}{\eta} + \eta K H^2 +HK\sqrt{d\log(dTm/\delta)}  \times \sqrt{\frac{dH\log (Tm/\delta)}{N}} \right) \\
\le & \log(AdTm/\delta)  \times \poly(H) \times  
\left( \frac{1}{\eta} + \eta K  +dK\sqrt{\frac{1}{N}} \right) 
    \end{aligned}
\end{equation}
where the second inequality  uses the fact that $R_\theta \le H\sqrt{d}$, $R_\phi=\lambda=1$.

Since our goal is to learn an $\epsilon$-optimal policy, we want to pick parameters $\eta$, $m$, $N$ and $K$ so that 
$\text{Regret}(K)/K$ is $\cO(\epsilon)$. By simple calculation, we can pick 
$$
\eta = \cO(\epsilon/C_H),~ K=\cO(\epsilon^{-2}/C_H) ~\text{and } N=d^2 \epsilon^{-2}/C_H
$$
where $C_H=\log^2(AdTm/\delta)  \times \poly(H)$.
% By picking $\eta=\sqrt{1/(KH)}$, we have 
% $$
% {\rm Regret}(T) 
% \le  \log^2(ATd/\delta)  \times \poly(H) \times 
% \cO\left( \sqrt{K}N +dK\sqrt{N} \right).
% $$
%  Recall that the total number of episodes is $T=KNH$, so we can pick $K=\sqrt{T}/d$ and $N=\sqrt{T}\times d$, which gives 
%  $$
%  {\rm Regret}(T)  \le 
% \log^2(ATd/\delta)  \times \poly(H) \times     \sqrt{d}\times
%   T^{3/4}.
%  $$



\begin{remark}
The proof also utilizes  some important observation of the independence between different steps $h\in[H]$, which I didn't explain in the  above proof sketch.
Please feel free to let me know if you have any difficulty following or reproducing the proof.
\end{remark}



\begin{lemma}
 [generalized policy-difference lemma, e.g., Lemma 1 in  \cite{shani2020optimistic}]\label{lem:pi-diff}
 For any policy $\pi$, 
 \begin{equation}
 \begin{aligned}
      V_1^\pi(s_1) - V_1^k (s_1)  
     = & \sum_{h=1}^H \E_{s_h\sim\pi} \left[\langle \pi_h(\cdot\mid s_h)- \pi^k_h(\cdot\mid s_h),  Q^k_h(s_h,\cdot)\rangle  \right] \\
     &- 
     \sum_{h=1}^H \E_{(s_h,a_h)\sim\pi} \left[Q_h^k(s_h,a_h) - r_h(s_h,a_h)- [\P_h V_{h+1}^k](s_h,a_h) \right].
     \end{aligned}
 \end{equation}
\end{lemma}




\begin{corollary}\label{cor:bonus}
With probability at least $1-\delta$, we have that for all $k\in[K]$
$$
\E_{\pi^k}[b_h^k(s_h,a_h)]
=  \tilde\cO\left(\sqrt{\frac{d^2}{N} }+  \frac{\sqrt{d} R_\phi}{\lambda}\sqrt{\frac{1}{N}}\right).
$$
\end{corollary}
\begin{proof}[Proof of Corollary \ref{cor:bonus}]
Consider a fixed $k\in[K]$ and let $k_0$ denote the largest integer no larger than $k$ such that $k_0 \% m =1$. 
If $k_0=k$, then 
the above relation immediately follows from the definition of $b_h^k$ and Proposition \ref{prop:optimism-upper-bound}. 
Otherwise, we can invoke Lemma \ref{lem:transfer} and \ref{lem:policy-stability} by noticing that 
(a) $\pi_h^k(a\mid s) \propto \pi_h^{k_0}(a\mid s) \times \exp(\eta \sum_{t=k_0}^{k-1} Q_h^t(s,a))$, (b) $k-k_0<m$ and (c) $m=\cO(1/(\eta H^2))$.
\end{proof}

\begin{lemma}[MD regret]\label{lem:md}
Suppose $\eta\le 1/H$. Then for all $(h,s,K)$ and $\mu\in\Delta_A$
$$
\sum_{k=1}^K\langle \mu - \pi^k_h(\cdot\mid s), \up{Q}^k_h(s,\cdot) \rangle = \cO\left( \frac{\log A}{\eta} + \eta K H^2 \right).
$$
\end{lemma}














\section{Supporting Lemmas}



\begin{lemma}[Concentration]\label{lem:concen}
 Suppose we sample $\cD:=\{(s_h^i,a_h^i,s_{h+1}^i)\}_{i=1}^n$ from an arbitrary policy. Let 
 \begin{itemize}
     \item $V_{h+1}:\cS\rightarrow [0,H]$ be a function independent of $\cD$,
     \item $\theta\in B_{H\sqrt{d}}(0)$ s.t. 
     $\langle \phi_h(s,a), \theta\rangle = r_h(s,a) + [\P_h V_{h+1}](s,a)$
     for all $(s,a)$,
     \item $\hat\theta = (\sum_{i=1}^n \phi^i{\phi^i}\trans + \lambda^2 \I_{d\times d})^{-1}\sum_{i=1}^m \phi^i [r^i+V_{h+1}^i]$ where $\phi_i:=\phi_h(s_h^i,a_h^i)$, $r^i:=r_h(s_h^i,a_h^i)$, and $V^i:=V_h(s_{h+1}^i)$.
 \end{itemize} 
 Then with probability $1-\delta$, we have that for any $(s,a)\in\cS\times\cA$:
 $$
 \left|\langle \theta-\hat\theta, \phi_h(s,a)\rangle \right|=  \left\| \phi_h(s,a)\right\|_{\left(\Cov+ \lambda^2 \I_{d\times d}\right)^{-1}} \times \cO\left(\sqrt{d\log(d/\delta)} +\lambda R_\theta\right). 
 $$
\end{lemma}
\begin{proof}
To simplify notations, denote $\Cov=\sum_{i=1}^n \phi^i{\phi^i}\trans$.  
\begin{equation}
    \begin{aligned}
    &\left|\langle\phi_h(s,a),  \theta-\hat\theta \rangle \right| \\
    = &\left|\left\langle\phi_h(s,a),   \left(\Cov + \lambda^2 \I_{d\times d}\right)^{-1}\left( \sum_i \phi^i [r^i+V^i] - \left(\Cov + \lambda^2 \I_{d\times d}\right)\theta \right) \right\rangle\right| \\
    \le & \left\| \phi_h(s,a)\right\|_{\left(\Cov+ \lambda^2 \I_{d\times d}\right)^{-1}} \times \left( \left\| \sum_i \phi^i [r^i+V^i-{\phi^i}\trans\theta]  \right\|_{\left(\Cov+ \lambda^2 \I_{d\times d}\right)^{-1}} + \lambda \left\|\theta \right\|_2
    \right) \\
    \le &  \left\| \phi_h(s,a)\right\|_{\left(\Cov+ \lambda^2 \I_{d\times d}\right)^{-1}} \times \left( \left\| \sum_i \phi^i \left[r^i+V^i-\E[r^i+V^i\mid s_h^i,a_h^i]\right]  \right\|_{\left(\Cov+ \lambda^2 \I_{d\times d}\right)^{-1}} + \lambda R_\theta
    \right) \\
    = &   \left\| \phi_h(s,a)\right\|_{\left(\Cov+ \lambda^2 \I_{d\times d}\right)^{-1}} \times \cO\left(\sqrt{d\log(d/\delta)} +\lambda R_\theta\right),
    \end{aligned}
\end{equation}
where the last relation holds with probability at least $1-\delta$ by standard vector concentration. 
\end{proof}

\begin{lemma}[Optimism]\label{lem:optimism} With probability at least $1-\delta$, for all $(h,s,k)\in[H]\times\cS\times[K]$:
$$
\begin{cases}
r_h(s_h,a_h)+ [\P_h V_{h+1}^k](s_h,a_h)  \le 
Q_h^{k}(s_h,a_h)\\
Q_h^{k}(s_h,a_h) \le 
r_h(s_h,a_h)+ [\P_h V_{h+1}^k](s_h,a_h) + 2 b_h^k(s_h,a_h),
\end{cases}
$$
where $b_h^k(s,a):= \left\| \phi_h(s,a)\right\|_{\left(\Cov+ \lambda^2 \I_{d\times d}\right)^{-1}} \times \cO\left(\sqrt{d\log(d/\delta)} +\lambda R_\theta\right)$.
\end{lemma}





==> legacy/prelim.tex <==
%!TEX root =  main.tex

\section{Preliminaries}


\paragraph{MDP.}
We consider the model of episodic Markov Decision Process (MDP).
Formally, an MDP  is defined by a tuple $(\cS,\cA,\P,R,H)$ where $\cS$ denotes the set of states, $\cA$ denotes the set of actions, $\P=\{\P_h\}_{h\in[H]}$ denotes the set of transition probability functions so that $\P_h(s'\mid s,a)$ is equal to the probability of transitioning to state $s'$ given that action $a$ is taken at state $s$ and step $h$, $R=\{R_h\}_{h\in[H]}$ denotes the collection of expected reward functions so that $R_h(s,a)$ is equal to the expected reward to receive if action $a$ is taken at state $s$ and step $h$, and $H$ denotes the length of each episode.  
An agent interacts an MDP in the form of episodes. Formally, we assume without loss of generality that each episode always starts from a \emph{fixed} initial state  $s_1$. 
At the $h\th$  step of this episode, the agent first observes the current state $s_h$, then takes action $a_h$ and receives reward $r_h(s_h,a_h)$ satisfying 
\[
\E[r_h(s_h,a_h) \mid s_h,a_h]=R_h(s_h,a_h)\,.
\] After that, the environment transitions to 
\[
s_{h+1}\sim \P_h(\cdot\mid s_h,a_h)\,. 
\]
The current episode terminates immediately once $r_H$ is received. 
Throughout this paper, we assume $\P$ and $R$ are unknown to the learner.


\paragraph{Linear MDP.}
A $d$-dimensional linear MDP \citep{jin2020provably} is defined by  two sets of feature mappings $\{\phi_h\}_{h\in[H]}\subseteq(\cS\times\cA\rightarrow \R^d)$, and $\{\psi_h\}_{h\in[H]}\subseteq(\cS\rightarrow \R^d)$ and a set of vectors $\{w^\star_h\}_{h\in[H]}\subseteq\R^d$ so that the transition probability functions can be represented as bilinear functions of feature mappings $\{\phi_h\}_{h\in[H]}$ and $\{\psi_h\}_{h\in[H]}$ and the reward functions can be represented as linear functions of $\{\phi_h\}_{h\in[H]}$. Formally, we have  that for all $(s,a,s')\in\cS\times\cA\times\cS$:
\begin{align*}
\begin{cases}
\P_h(s'\mid s,a) 
 = \langle \phi_h(s,a), \psi_h(s')\rangle, \quad \\
R_h(s,a) =\langle \phi_h(s,a), w^\star_h\rangle.
\end{cases}
\end{align*}
For the purpose the regularity, linear MDPs also require that 
$$
\max_{h,s,a}\|\phi_h(s,a)\|_2 \le 1,  \quad \max_h \|w^\star_h\|_2 \le \sqrt{d},
$$
and for any function $V_{h+1}:\cS\rightarrow[0,1]$, 
$$
\int_{s\in\cS}V_{h+1}(s) \psi_{h+1}(s) ds \le \sqrt{d}.
$$
Throughout this paper, we assume only $\{\phi_h\}_{h\in[H]}$ is available to the learner while 
$\{\psi_h\}_{h\in[H]}$ and 
$\{w^\star_h\}_{h\in[H]}$ are not.


\paragraph{Policy and value.} 

A (Markov) policy is a set of conditional probability functions $\pi=\{\pi_h\}_{h\in[H]}$ so that  $\pi_h(\cdot\mid s)\in\Delta_\cA$ gives the distribution over the action set conditioning on the current state $s$ at step $h$.
We define the V-value functions of policy $\pi$ by $\{V^\pi_h\}_{h\in[H]}\subseteq (\cS\rightarrow \R)$ so that $V_h^\pi(s)$ is equal to the expected cumulative reward an agent will receive if she follows policy $\pi$ starting from state $s$ and step $h$. Formally, 
$$
V^\pi_h(s):= \E\left[ \sum_{h'=h}^H r_{h'}(s_{h'},a_{h'})\mid s_h=s, a_{h'}\sim \pi_{h'}(s_{h'}) \right],
$$
where the expectation is with respect to the randomness  of the transition, the reward and the policy. Similarly, we can define the Q-value functions of policy $\pi$ by $\{Q^\pi_h\}_{h\in[H]}\subseteq (\cS\times\cA\rightarrow \R)$ so that $Q_h^\pi(s,a)$ is equal to the expected cumulative reward an agent will receive if she follows policy $\pi$ starting from taking action $a$ at state $s$ and step $h$. Formally, 
\begin{align*}
Q^\pi_h(s,a)
& := \E\Biggl[ \sum_{h'=h}^H r_{h'}(s_{h'},a_{h'})\mid  \\
& \qquad \qquad 
(s_h,a_h)=(s,a), a_{h'}\sim \pi_{h'}(s_{h'}) \Biggr].
\end{align*}
We denote by $\pi^\star=\{\pi^\star_h\}_{h\in[H]}$ the optimal policy such that $\pi^\star  \in \argmax_\pi V^\pi_h(s)$ for all $(s,h)\in\cS\times[H]$.
By backward induction, one can easily prove that there always exists an optimal Markov policy. For simplicity of notations, we denote by $V^\star_h:=V^{\pi^\star}_h$ and $Q^\star_h:=Q^{\pi^\star}_h$ the optimal value functions. Note that given an MDP, the optimal value functions are unique despite that there may exist multiple optimal policies.


\paragraph{Learning objective.} 
The objective of this paper is to design an efficient policy optimization algorithm to  learn an $\epsilon$-optimal policy $\pi$ such that $V^\pi_1(s_1)\ge V^\star_1(s_1)-\epsilon$.
Here the optimality is only  measured by the value at the initial state $s_1$,  because (a) each episode always starts from $s_1$, and (b) this paper  studies the online exploration setting without access to a simulator, which means some states might be unreachable and learning optimal policies starting from those state is in general impossible. 

==> legacy/proof_sketch.tex <==
%!TEX root =  main.tex
\section{Proof of Theorem \ref{thm:main}}
\label{sec:proof-sketch}
In this section, we prove Theorem \ref{thm:main}. 
The proofs of the lemmas used in this section can be found in  Appendix \ref{app:linear}.

Recall in Algorithm \ref{alg:oppo}, 
$\piout$ is sampled uniformly at random from $\{\pi^k\}_{k\in[K]}$, so we have 
\begin{align*}
%\begin{aligned}
% \MoveEqLeft
    \lefteqn{\E\left[V^\star_1(s_1) - V_1^{\piout}(s_1)\right]} \\
    & = \frac{1}{K}\sum_{k=1}^K \left[V_1^\star(s_1)-V_1^{\pi^k}(s_1) \right] \\
    & =   
    \underbrace{\frac{1}{K}\sum_{k=1}^K \left[V_1^\star(s_1)-\oV_1^{k}(s_1) \right]}_{\rm \textbf{Term (I)}} \\
    &\qquad+   \underbrace{\frac{1}{K}\sum_{k=1}^K \left[\oV_1^{k}(s_1)-V_1^{\pi^k}(s_1) \right]}_{\rm\textbf{ Term (II)}}.
%       \end{aligned}
\end{align*}
\paragraph{Term (I).} To begin with, we import the following generalized  policy difference lemma from \citep{shani2020optimistic,cai2020provably}.
\begin{lemma}
 [generalized policy-difference lemma]\label{lem:pi-diff}
 For any policy $\pi$ and $k\in[K]$, 
 \begin{equation*}
 \begin{aligned}
% \MoveEqLeft      
V_1^\pi&(s_1) - \oV_1^k (s_1) \\ 
     =  & \sum_{h=1}^H \E_{s_h\sim\pi} \left[\langle \pi_h(\cdot\mid s_h)- \pi^k_h(\cdot\mid s_h),  \oQ^k_h(s_h,\cdot)\rangle  \right] \\
     &- 
     \sum_{h=1}^H \E_{(s_h,a_h)\sim\pi} \Biggl[\oQ_h^k(s_h,a_h) - R_h(s_h,a_h)\\
     & \quad\quad\quad\quad\quad\quad - \E_{s_{h+1}\sim\P(\cdot \mid s_h,a_h)}\Bigl[ \oV_{h+1}^k(s_{h+1})\Bigr] \Biggr].
     \end{aligned}
 \end{equation*}
\end{lemma}
By invoking Lemma \ref{lem:pi-diff} with $\pi=\pi^\star$, we have 
\begin{equation}\label{eq:1}
\begin{aligned}
    &{\rm Term (I)} 
    = \frac{1}{K}\sum_{k=1}^K\left[
      V_1^\pi(s_1) - \oV_1^k (s_1)  \right]\\
     &\le  H\max_{h,s} \left[\frac{1}{K}\sum_{k=1}^K\left\langle \pi_h^\star(\cdot\mid s)- \pi^k_h(\cdot\mid s),  \oQ^k_h(s,\cdot)\right\rangle  \right] \\
     &\quad+ H\max_{h,s,a}
     \Biggl[ R_h(s,a)+ \E_{s'\sim\P(\cdot \mid s,a)}\left[ \oV_{h+1}^k(s')\right]\\
     &\qquad \qquad  -\oQ_h^k(s,a)  \Biggr] \\
     & \le  \cO\left( \frac{H\log |\cA|}{\eta K} + \eta  H^3\right) +H\max_{h,s,a}
     \Biggl[ R_h(s,a)+ \\
      & ~\qquad\qquad\qquad \E_{s'\sim\P(\cdot \mid s,a)}\left[ \oV_{h+1}^k(s')\right] 
       -\oQ_h^k(s,a)  \Biggr],
     \end{aligned}
\end{equation}
where the second inequality follows from the standard regret bound of online mirror ascent.
To control the second term on the RHS of Equation \eqref{eq:1}, we introduce the following lemma showing that $\oQ_h^k$ is an optimistic estimate of $R_h(s,a)+ \E_{s'\sim\P(\cdot \mid s,a)}\left[ \oV_{h+1}^k(s')\right]$ and the degree of over-optimism can be bounded by the bonus function. 

\begin{lemma}[optimism of value estimates]\label{lem:opt} Under the same choice of $\lambda$ and $\alpha$ as in Theorem \ref{thm:main}, with probability at least $1-\delta$: for all $(k,h,s,a)\in[K]\times[H]\times\cS\times\cA$:
\begin{equation*}
    \begin{aligned}
 0\le\, &\oQ_h^k(s,a)-R_h(s,a) \\
 &- \E_{s'\sim\P(\cdot \mid s,a)}\left[ \oV_{h+1}^k(s')\right]\le 2 b_h^k(s,a),
\end{aligned}
\end{equation*}
where $\{b_h^k\}_{h\in[H]}$ are the bonus functions used in \lspe$(\pi^k,\cD^k,\lambda,\alpha)$ for computing $\{\oQ_h^k\}_{h\in[H]}$.
\end{lemma}
Importantly,  Lemma \ref{lem:opt} holds with a bonus function that  is  smaller by a factor of $\sqrt{d}$ than the typical one used in linear function approximation \citep[e.g.,][]{jin2020provably}, which is key to obtaining the optimal dimension dependence. The main reason that this smaller bonus function suffices is that we recollect fresh samples every $m$ iterations and split the data (Line \ref{line:split} in Algorithm \ref{alg:lspe}) to eliminate the correlation between different steps $h\in[H]$.
By combining Lemma \ref{lem:opt} with Equation \eqref{eq:1}, we obtain
\begin{equation*}
    {\rm Term (I)}\le  \cO\left( \frac{H\log |\cA|}{\eta K}+\eta H^3\right).
\end{equation*}

\paragraph{Term (II).} By repeatedly applying the second inequality in Lemma \ref{lem:opt}, the definition of $\oV^k$ and the Bellman equation under policy $\pi^k$, one can easily show 
$\oV_1^{k}(s_1)-V_1^{\pi^k}(s_1)
\le 2\sum_{h=1}^H \E_{\pi^k}[b_h^k(s_h,a_h)]$, which implies 
\begin{equation}\label{eq:2}
    {\rm Term (II)} \le 
    2\max_{k\in[K]}\sum_{h=1}^H \E_{\pi^k}[b_h^k(s_h,a_h)].
\end{equation}
Denote by $t_k$ the index of the last iteration of collecting fresh data before the $k\th$ iteration. By exploiting the softmax parameterization structure of $\{\pi^k\}_{k\in[K]}$, one can show that the visitation measure over state-action pairs induced by executing  policy $\pi^k$ is actually very close to the one induced by $\pi^{t_k}$ in the following sense.
\begin{lemma}[policy Lipschitz]\label{lem:pi-close}
Suppose we choose $\eta$ and $m$ such that $\eta m \le 1/H^2$, then for any $k\in\mathbb{N^+}$ and any function $f:\cS\times\cA\rightarrow \R^+$:
$$
\E_{\pi^k}[f(s_h,a_h)] = \Theta\left(
\E_{\pi^{t_k}}[f(s_h,a_h)]\right).
$$
\end{lemma}
Combining Lemma \ref{lem:pi-close} with Equation \eqref{eq:2}, we have 
$${\rm Term (II)} \le 
    \cO\bigg(\max_{k\in[K]}\sum_{h=1}^H \E_{\pi^{t_k}}[b_h^k(s_h,a_h)]\bigg).
    $$
Now recall that the bonus function $b_h^k$ is defined by using the dataset $\cD^{t_k}$ collected exactly from executing policy $\pi^{t_k}$, which implies that its expectation under $\pi^{t_k}$ should be rather small when the batch size $N$ is large enough, as formalized in the following lemma. 


\begin{lemma}[on-policy uncertainty] \label{lem:on-policy-bonus}
Let $\pi$ be an arbitrary policy and $\lambda \ge 1$. % replaced B_\phi^2 with 1
Suppose we sample $\{(s_h^n,a_h^n)\}_{n=1}^N$ i.i.d. from $\pi$. Denote $\Sigma_h=\sum_{i=1}^{N} \phi_h(s_h^i,a_h^i) \phi_h\trans(s_h^i,a_h^i)$. 
Then with  probability at least $1-\delta$:
\begin{equation*}
\begin{aligned}
    &\E_{(s_h,a_h)\sim\pi}\big[\|\phi_h(s_h,a_h)\|_{(\Sigma_h+ \lambda  \I_{d\times d})^{-1}}\big] \\
& \qquad\qquad\qquad= \cO\left(\sqrt{\frac{d\log (N/\delta)}{N} }\right).
\end{aligned}
\end{equation*}
\end{lemma}
As a result, by Lemma \ref{lem:on-policy-bonus} and the definition of $b_h^k$, we have that with  probability at least $1-\delta$: for all $k\in[K]$, 
$$
\sum_{h=1}^H \E_{\pi^{t_k}}[b_h^k(s_h,a_h)] = {\cO}\left( Hd\sqrt{\frac{H\log^2(KN/\delta)}{N}}\right),
$$
which implies 
$$
{\rm Term (II)}\le {\cO}\left( \sqrt{\frac{d^2 H^3\log^2(KNH/\delta)}{N}}\right).
$$
Finally, we complete the entire proof by combining all pieces together with a union bound and plugging in a sufficiently small constant $\delta$, along with the choice of $K,m,\eta$ and   $N$.


\section{Proof of Theorem \ref{thm:tabular}}
\label{sec:tab}


The proof of Theorem \ref{thm:tabular} follows basically the same as that of Theorem \ref{thm:main}. The only modification needed is to replace Lemma \ref{lem:opt} and \ref{lem:on-policy-bonus} by their tabular counterparts, which we state below. 

\begin{lemma}[optimism of value estimates: tabular]\label{lem:opt-tabular} Under the same choice of $\alpha$ as in Theorem \ref{thm:tabular}, with probability at least $1-\delta$: for all $(k,h,s,a)\in[K]\times[H]\times\cS\times\cA$:
\begin{equation*}
    \begin{aligned}
 0\le\, &\oQ_h^k(s,a)-R_h(s,a) \\
 &- \E_{s'\sim\P(\cdot \mid s,a)}\left[ \oV_{h+1}^k(s')\right]\le 2 b_h^k(s,a),
\end{aligned}
\end{equation*}
where $\{b_h^k\}_{h\in[H]}$ are the bonus functions used in \pe$(\pi^k,\cD^k,\alpha)$ for computing $\{\oQ_h^k\}_{h\in[H]}$.
\end{lemma}



\begin{lemma}[on-policy uncertainty: tabular] \label{lem:on-policy-bonus-tabular}
Let $\pi$ be an arbitrary policy. % replaced B_\phi^2 with 1
Suppose we sample $\{(s_h^n,a_h^n)\}_{n=1}^N$ i.i.d. from $\pi$. Denote $J_h(s,a)=\sum_{i=1}^{N} \mathbf{1}((s_h^i,a_h^i)=(s,a))$. 
Then with  probability at least $1-\delta$:
\begin{equation*}
\begin{aligned}
    \E_{(s_h,a_h)\sim\pi}\left[\sqrt{\frac{1}{J_h(s,a)+1}}\right] = \cO\left(\sqrt{\frac{SA\log (N/\delta)}{N} }\right).
\end{aligned}
\end{equation*}
\end{lemma}

The proofs of Lemma \ref{lem:opt-tabular} and \ref{lem:on-policy-bonus-tabular} can be found in Appendix \ref{app:tab}.
